Adaptive Hypergraph Network for Trust Prediction

Trust plays an essential role in an individual's decision-making. Traditional trust prediction models rely on pairwise correlations to infer potential relationships between users. However, in the real world, interactions between users are usually complicated rather than pairwise only. Hypergraphs offer a flexible approach to modeling these complex high-order correlations (not just pairwise connections), since hypergraphs can leverage hyperedeges to link more than two nodes. However, most hypergraph-based methods are generic and cannot be well applied to the trust prediction task. In this paper, we propose an Adaptive Hypergraph Network for Trust Prediction (AHNTP), a novel approach that improves trust prediction accuracy by using higher-order correlations. AHNTP utilizes Motif-based PageRank to capture high-order social influence information. In addition, it constructs hypergroups from both node-level and structure-level attributes to incorporate complex correlation information. Furthermore, AHNTP leverages adaptive hypergraph Graph Convolutional Network (GCN) layers and multilayer perceptrons (MLPs) to generate comprehensive user embeddings, facilitating trust relationship prediction. To enhance model generalization and robustness, we introduce a novel supervised contrastive learning loss for optimization. Extensive experiments demonstrate the superiority of our model over the state-of-the-art approaches in terms of trust prediction accuracy. The source code of this work can be accessed via https://github.com/Sherry-XU1995/AHNTP.

==> secs/0.abs.tex <==
\begin{abstract}
Trust plays an essential role in an individual's decision-making. Traditional trust prediction models rely on pairwise correlations to infer potential relationships between users. However, in the real world, interactions between users are usually complicated rather than pairwise only. Hypergraphs offer a flexible approach to modeling these complex high-order correlations (not just pairwise connections), since hypergraphs can leverage hyperedeges to link more than two nodes. However, most hypergraph-based methods are generic and cannot be well applied to the trust prediction task. In this paper, we propose an Adaptive Hypergraph Network for Trust Prediction (AHNTP), a novel approach that improves trust prediction accuracy by using higher-order correlations. AHNTP utilizes Motif-based PageRank to capture high-order social influence information. In addition, it constructs hypergroups from both node-level and structure-level attributes to incorporate complex correlation information. Furthermore, AHNTP leverages adaptive hypergraph Graph Convolutional Network (GCN) layers and multilayer perceptrons (MLPs) to generate comprehensive user embeddings, facilitating trust relationship prediction. To enhance model generalization and robustness, we introduce a novel supervised contrastive learning loss for optimization. Extensive experiments demonstrate the superiority of our model over the state-of-the-art approaches in terms of trust prediction accuracy. The source code of this work can be accessed via https://github.com/Sherry-XU1995/AHNTP.
\end{abstract}

\begin{IEEEkeywords}
Hypergraph, Contrastive Learning, Trust Prediction
\end{IEEEkeywords}

==> secs/1.intro.tex <==
\section{Introduction}
Trust is characterized as an inclination to rely on others, and it represents a recognition of the trustworthiness of a person \cite{rotter1971generalized}. Trust can also be described as an individual's willingness to be influenced by the actions of another person \cite{mayer1995integrative}. Trust relationships in social networks have a significant influence on many aspects of people's lives, \ieno, people's decision-making, product recommendations, financial institutions' assessment of customer credit risk, \etcno. In a social network, for instance, if a user wants to purchase a tennis racket but is unsure which brand to choose, recommendations from trusted friends, favorite athletes, or internet celebrities can greatly impact his/her decision. This illustrates the importance of trust in purchase decisions. From a merchant's perspective, understanding the trust relationships between customers can enhance their ability to identify potential customers. However, in real scenarios of social networks, users are usually unknown to each other and it is difficult to observe explicit trust relationships. In this situation, users can still establish an implicit trust relationship based on the characteristics of trust inference \cite{xu2022attention}. For example, users may trust individuals who share similar interests, even if no direct interactions between them. Trust prediction in social networks leverages user behavior data to predict these implicit trust relationships, typically incorporating various features such as historical transaction records, social network connections, and personal profiles\cite{abdullah2017retweet, lin2020guardian, meo2019trust, ghafari2020survey}.


In the literature, trust prediction methods in social networks can be divided into three categories: (1) propagation-based methods, (2) matrix-based methods, and (3) Graph Neural Network (GNN)-based methods. Propagation-based methods are based on trust propagation rules in social networks. Matrix-based methods predict trust connections between non-adjacent users using various factors, including historical user behavior and personal preferences. However, they often neglect the structure information of the network. In contrast to the two categories, GNN-based methods have shown promise in modeling relational data \cite{wu2020comprehensive}, and thus they have been adopted in trust prediction. For example, the DeepTrust model proposed by Wang et al. \cite{wang2019deeptrust} adopts a deep pairwise neural network to capture the latent features of users from their ratings and reviews on trust prediction. However, it only considers the information of directly connected nodes but does not consider the structure of the networks. Liu et al. \cite{liu2019neuralwalk} design a neural network, NeuralWalk, where they consider indirectly connected nodes to solve the multi-hop trust assessment problem. Furthermore, the model proposed by Lin et al. \cite{lin2020guardian} can learn the rule of trust propagation and aggregation in online social networks with better efficiency than NeuralWalk using GCN. The lack of user features and the difficulties in dealing with multi-aspect properties of social trust limit the capability of the model. Furthermore, to address this problem, Jiang et al. \cite{jiang2022gatrust} develop the GATrust model, which adopts both graph attention networks (GAT) \cite{velickovic2017graph} and GCN to learn the various latent factors of both trustor and trustee.




\begin{figure}[t]
  \centering
  \begin{minipage}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{3.png}
    \caption{High-order correlation among users and items.}
    \label{fig 2}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\linewidth}
    \includegraphics[width=\linewidth]{22.png}
    \caption{The following relation between five users.}
    \label{fig 1}
  \end{minipage}
\end{figure}


However, most of these GNN-based trust prediction methods cannot directly capture high-order correlations between users. Here, the\textit{ high-order correlation} refers to dependencies that involve more than two nodes rather than simple pairwise correlations \cite{gao2022hgnn}.  For example, in Fig. \ref{fig 2}, Users 1, 2, and 3 share an interest in swimming, and Users 2 and 4 are alumni of the same school. In addition to the pairwise correlations between user-hobby and user-school, there also exist high-order correlations: Users 1, 2, and 3, based on their shared hobby, and Users 2 and 4, according to their school affiliation. These high-order correlations among users are in the pattern of the group, reflecting the information from the social community or social circle. As indicated in social science \cite{cui2018trust}, users have the tendency to maintain a high level of trust in such a specific circle. Incorporating these high-order correlations can produce a more comprehensive embedding, resulting in more accurate trust prediction outcomes. However, representing these high-order correlations effectively in a traditional graph is a challenge. 


Firstly, traditional GNN-based methods face difficulties when dealing with isolated nodes. These methods extract user features from pairwise interactions among user-user pairs. They can only capture long-range dependencies in relations (high-order correlation), such as the transitivity of friendship, by aggregating information from neighboring nodes through multiple layers of neural networks \cite{yu2021self}. In the context of online social networks, a prevalence of isolated nodes is observed \cite{guan2023sparse}. Since GNN-based methods heavily depend on pairwise correlation, these isolated nodes can hardly be updated during the learning process. Therefore, they cannot effectively and accurately embed this critical information, which subsequently affects the performance of trust prediction \cite{guan2023sparse}. 

Secondly, GNN-based models face challenges in capturing triangular high-order user relation patterns. For example, as shown in Fig. \ref{fig 1}, the triangular connection among Users 1, 2, and 3 introduces a high-order correlation. These high-order triangle correlations are prevalent and can often convey crucial information in the trust prediction of social networks. Many existing methods primarily focus on first-order pairwise correlations in analyzing the influence of individuals. As shown in Fig. \ref{fig 1}, there are five users, and the edge $e_{ij}$ refers to the directed connection between Users $i$ and $j$. $e_{13}$ indicates User 1 follows User 3. In a traditional graph, the same value is assigned to the original weight of $e_{15}$ and $e_{13}$. However, as observed in Fig. \ref{fig 1}, User 1 has a closer relationship with User 3 than User 5. This is because User 1 follows both User 2 and User 3, while User 2 and User 3 are friends as well. 
\begin{figure}[t]  
	\begin{center}
	\includegraphics[width=2.0in]{13.png}
	\end{center}
	\caption{The comparison between graph and hypergraph.}
	\label{fig 13}
\end{figure}Therefore, we should not set the equal weight for $e_{15}$ and $e_{13}$, since Users 1 and 3 co-occur within this triangular structure. Instead, the weight assigned to $e_{13}$ should be higher than that of $e_{15}$. Therefore, the high-order triangular structures of social influence should be considered when predicting trust relationships.




Hypergraphs \cite{bretto2013hypergraph} can deal with high-order correlations by using hyperedges to connect more than two nodes. This structure can model complex and high-order correlations. As shown in Fig. \ref{fig 13}(a), in a general graph structure, each edge can only connect two nodes. In contrast, as depicted in Fig. \ref{fig 13}(b), in a hypergraph, its hyperedge can link multiple nodes simultaneously, which extends the graph structure to a more comprehensive nonlinear space. A hyperedge can be constructed from various aspects, such as the attribute cluster and the community. High-order correlations can be directly presented on the hyperedge instead of a long message-passing chain in traditional GNN-based methods. Therefore, this approach provides a robust framework for capturing multivariate relationships and high-dimensional data. However, current hypergraphs \cite{bretto2013hypergraph, gao2022hgnn, feng2019hypergraph} are not specifically tailored for trust prediction tasks. Specifically, in the context of social trust prediction, these models face the following three limitations. 
 






% \textit{The first limitation} is that trust prediction is inherently linked to complex social relationships and factors. Social factors like social reputation, particularly in relation to individuals possessing significant social influence, are often overlooked in hypergraph-based models. \textit{The second limitation} is about the fluctuating nature of trust levels, which can vary with changes in the environment or among the individuals involved. Hypergraph-based models cannot effectively distinguish these varying influences toward different user pairs. \textit{The third limitation} involves the hypergraph-based methods themselves, which often overlook the issues of potential information loss and distortion that may occur during the process of graph reconstruction. 



 
 \textit{The first limitation} is that they do not fully consider the social influence of users. The significant role of social influence in trust prediction has been reported in \cite{leskovec2013status, caverlee2008socialtrust, wang2015modeling, tang2016transfer}. The opinions and behaviors of individuals with high social influence, such as internet celebrities or domain experts, tend to have significant influences on social networks. Their suggestions or opinions are more likely to be accepted or trusted by other people \cite{tang2016transfer}. Therefore, the important influence of these high-social-influence people should be considered in the prediction of trust.

\textit{The second limitation} is to distinguish the different influences of hyperedges on different pairs of users. Most of the hypergraph-based methods \cite{feng2019hypergraph, gao2022hgnn, yadati2019hypergcn} rely on a weight matrix to determine the impact of features on output. However, these weights are typically static and uniformly shared across all user pairs, which means they keep constant regardless of the different concerns of users in trust establishment. This approach limits the ability of the model to capture complex and dynamic interactions between users. In the real world, different users can have different concerns in trust establishment. For example, common hobbies might be the key factor in building trust for some users, while for others, similar educational backgrounds might play a more crucial role. Therefore, it's necessary to dynamically adjust the weights of the influential factors based on the specific situation of each user pair. HyperGAT \cite{bai2021hypergraph} has been proposed to incorporate a graph attention mechanism to identify these different influential factors. However, this method requires transforming hyperedges into a homogenous domain of nodes before training. This process may not be able to accurately capture the distinct user interactions. 

\textit{The third limitation} is the loss function of existing methods. Most of those methods utilize cross-entropy loss as their loss function. However, according to the study in \cite{zhang2018generalized}, the use of cross-entropy loss can affect the robustness when dealing with noisy labels. Specifically, when training data contains errors or noisy labels, cross-entropy loss may be sensitive to these labels, which can lead to the overfitting problem. In addition, cross-entropy loss can also lead to the possibility of poor margins \cite{elsayed2018large}, resulting in less distinct boundaries between classes. This can affect the performance, particularly when dealing with datasets characterized by class imbalances. Hence, it is significant to devise a novel loss function that addresses the limitations associated with cross-entropy loss.


 
To address the limitations mentioned above, we propose a novel Adaptive Hypergraph Network for Trust Prediction (AHNTP). To address the first limitation, we integrate the social influence factor (e.g.,  the triangular motifs in social networks) into the hypergraph structure to capture the high-order correlation in the social network. To address the second limitation, we employ an adaptive Graph Convolutional Network (GCN) to effectively aggregate user information and dynamically identify social influence factors. To address the third limitation, we introduce the contrastive learning method. Specifically, our model utilizes a Motif-based PageRank algorithm \cite{zhao2018ranking} to capture social influence information. It enables the consideration of high-order relationships within specific triangular interactions present in social interactions. Subsequently, we establish a two-tier hypergroup framework. One is based on node-level attributes and the other is based on structure-level attributes. The hypergroup represents a collection of nodes linked by specific correlations. On the basis of different types of correlation, we establish different hypergroups. This approach not only facilitates capturing the correlations but also effectively handles diverse data types and features. In addition, by adopting an adaptive hypergraph GCN, we can dynamically differentiate the influence of each hyperedge on trust evaluation and obtain an accurate representation of users. Finally, we incorporate contrastive learning to improve the generalization and robustness of the model. Experiments on two real datasets have illustrated that AHNTP outperforms state-of-the-art methods in trust prediction. Our contributions are summarized as follows.

\begin{itemize}
    \item[(1)] Firstly, we design a comprehensive and adaptive hypergraph model AHNTP, which can capture the high-order correlation and handle diverse data types and features in trust prediction. 
    \item[(2)] Secondly, we incorporate motif-based PageRank into hypergraphs, which allows us to identify users who have high social influence. In addition, we introduce a multi-hop hypergroup to consider the property of trust propagation. Therefore, our model can embed accurate information of social relationships. 
    \item[(3)] Thirdly, we utilize an adaptive GCN module to distinguish the dynamic impact of different factors on trust prediction. This allows our model to assign higher priority to relevant factors and disregard redundant ones, thereby improving the learning capability of the model.
    \item[(4)] Fourthly, we employ a supervised contrastive learning method to optimize the training loss, which reduces the distances between users with high similarity and increases the distances for those with low similarity.
    \item[(5)] Extensive experiments have been conducted on real-world datasets. The results have demonstrated the proposed AHNTP can outperform the state-of-the-art methods in terms of trust prediction accuracy.
   
\end{itemize}
